Curvilinear Mesh Adaptation using Radial Basis Function Interpolation and Smoothing

We present a new iterative technique based on radial basis function (RBF) interpolation and smoothing for the generation and smoothing of curvilinear meshes from straight-sided or other curvilinear meshes. Our technique approximates the coordinate deformation maps in both the interior and boundary of the curvilinear output mesh by using only scattered nodes on the boundary of the input mesh as data sites in an interpolation problem. Our technique produces high-quality meshes in the deformed domain even when the deformation maps are singular due to a new iterative algorithm based on modification of the RBF shape parameter. Due to the use of RBF interpolation, our technique is applicable to both 2D and 3D curvilinear mesh generation without significant modification.

==> def.tex <==

% ++++ Vectors
\def \vepsilon{ \boldsymbol{\varepsilon} }
\def \vu{ \boldsymbol{u} }
\def \vU{ \boldsymbol{U} }
\def \vzeta{ \boldsymbol{\zeta} }
\def \vx{ \boldsymbol{x} }
\def \vp{ \boldsymbol{p} }
\def \vs{ \boldsymbol{s} }
\def \vn{ \boldsymbol{n}}
\def \vf{ \boldsymbol{f} }

\def \Hx { \hat{1} }
\def \Hy { \hat{2} }
\def \Ht{ \hat{t} }
\def \Hu{ \hat{u} }
\def \Hv{ \hat{v} }
\def \Hw{ \hat{w} }
\def \vc { \boldsymbol{c} }

\def \vn{ \boldsymbol{n} }
\def \vW{ \boldsymbol{W} }
\def \vv{ \mathbf{v} }

\def \vsig{ \boldsymbol{\sigma}}
\def \tnsrsig{ \underset{\thickapprox}{\boldsymbol{\sigma} }}
\def \tnsreps{\underset{\thickapprox}{\boldsymbol{\varepsilon} }}

%  +++++ Tensors
\def \tnsrsig{ \underset{\thickapprox}{\boldsymbol{\sigma} }}
\def \tnsreps{\underset{\thickapprox}{\boldsymbol{\varepsilon} }}
%  +++++ Operators
\def\calB{{\mathcal B}}
\def\calF{{\mathcal F}}
\def\calU{{\mathcal U} }
\def\calUvu{ \mathcal U(\vu) }
\def\calR{\mathcal R }
\def\calS{{ \mathcal S}}
\def\calE{{ \mathcal E}}
\def\calD{{ \mathcal D}}
\def\calP{{ \mathcal P}}
\def\calI{{ \mathcal I}}
\def\calG{{ \mathcal G}}

\def \vX{ \mathbf{x} }
\def \vY{ \mathbf{y} }
\def \vg{ \mathbf{g} }

%**************************************
\newcommand{\alp}[3]{{\left . \alpha_{#1} \right |^{#2}_{#3}\ }}
\newcommand{\bet}[3]{{\left .  \beta_{#1} \right |^{#2}_{#3}\ }}
\newcommand{\Balp}[3]{{\left . \BM {\alpha}_{#1} \right |^{#2}_{#3}\ }}
\newcommand{\Bbet}[3]{{\left . \BM {\beta}_{#1} \right |^{#2}_{#3}\ }}
\newcommand{\Bzet}[2]{{\BM {\zeta}^{#1}_{#2}}}
\newcommand{\B}[1]{{\underline{#1}}}
\newcommand{\Bf}[1]{\boldsymbol{#1}}
\newcommand{\Bc}[1]{\mathcal{#1}}
\newcommand{\Bd}[1]{\mathbb{#1}}
\newcommand{\Bs}[1]{\mathsf{#1}}
\newcommand{\dif}{\mathrm{d}}
\newcommand{\pdif}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\pfrac}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\scite}[1]{\textsuperscript{\cite{#1}}}
\newcommand{\ul}{\underline}
\newcommand{\II}{\ensuremath{I \hspace{-0.2em} I}}
\newcommand{\III}{\ensuremath{I \hspace{-0.2em} I \hspace{-0.2em} I}}
\newcommand{\CI}{\mathbf{C} \hspace{-0.6em} \mbox{\small I} }
\newcommand{\ci}{\mathbf{c} \hspace{-0.6em} \mbox{\small I} }
\newcommand{\ljump}{\left [  \hspace{-0.21em} \left | }
\newcommand{\rjump}{\right | \hspace{-0.21em} \right ]}
\newcommand{\odif}[2]{\frac{\mathrm{d}  {#1}}{\mathrm{d} {#2}}}
\newcommand{\into}{ \int_{\Omega}}
\newcommand{\difo}{ \;\mathrm{d}\Omega}
\newcommand{\difg}{ \;\mathrm{d}\Gamma}
\newcommand{\BM}[1]{\mbox{\boldmath $#1$}}
\newcommand{\BMB}[1]{\mbox{$\mathbb #1$}}
%\newcommand{\BM}[1]{\mbox{$\mathbf  #1$}}
\newcommand{\bdiff}{\BM{\cal D}}
\newcommand{\diff}{{\cal D}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Nel}{N_{el}}
\newcommand{\smfrac}[2]{\mbox{$\frac{#1}{#2}$}}


\newcommand{\lon}{\lambda}
\newcommand{\lat}{\theta}
\newcommand{\lond}{\lambda}
\newcommand{\latd}{\theta}
\newcommand{\lons}{\lambda^{\rm e}}
\newcommand{\lats}{\theta^{\rm e}}
\newcommand{\lf}{\left}
\newcommand{\rt}{\right}
\newcommand{\lp}{\lf (}
\newcommand{\rp}{\rt )}
\newcommand{\ep}{\varepsilon}
\newcommand{\tngt}{\boldsymbol{\tau}}
\newcommand{\utngt}{\hat{\boldsymbol{\tau}}}
\newcommand{\unrml}{\hat{\boldsymbol{\eta}}}
\newcommand{\frc}{\mathbf{F}}
\newcommand{\matlab}{\textsc{Matlab\;}}

\def \Xd{ X^{\rm d} }
\def \Xs{ X^{\rm s} }
\def \Yd{ Y^{\rm d} }
\def \Ys{ Y^{\rm s} }
\def \vXd{ \boldsymbol{X}^{\rm d} }
\def \vXs{ \boldsymbol{X}^{\rm s} }
\def \ucd{ \vec{\alpha}^X_{\rm d} }
\def \ucdb{ \vec{\alpha}^Y_{\rm d} }
\def \uXd{ \vec{X}_{\rm d}(t) }
\def \uvXd{ \vec{\vX}_{\rm d} }
\def \uvXs{ \vec{\vX}_{\rm s} }
\def \uYd{ \vec{Y}_{\rm d}(t) }
\def \uXs{ \vec{X}_{\rm s}(t) }

% ++++ Vectors.
\def \vepsilon{ \boldsymbol{\varepsilon} }
\def \vu{ \boldsymbol{u} }
\def \vU{ \boldsymbol{U} }
\def \vzeta{ \boldsymbol{\zeta} }
\def \vx{ \boldsymbol{x} }
\def \va{ \boldsymbol{a} }
\def \vy{ \boldsymbol{y} }
\def \vn{ \boldsymbol{n}}
\def \vt{ \boldsymbol{t}}
\def \vf{ \boldsymbol{f} }
%\def \vX{ \boldsymbol{X} }
\def \vc{ \mathbf{c} }
\def \vd{ \mathbf{d} }
\def \vP{ \boldsymbol{P} }
\def \vB{ \boldsymbol{B} }
\def \vp{ \boldsymbol{p} }
\def \vF{ \boldsymbol{F} }

\def \vs{ \mathbf{s}}

\def \Hx { \hat{1} }
\def \Hy { \hat{2} }
\def \Ht{ \hat{t} }
\def \Hu{ \hat{u} }
\def \Hv{ \hat{v} }
\def \Hw{ \hat{w} }
\def \Htau{ \hat{\tau} }
\def \vhtau{ \boldsymbol{\Htau} }
\def \vc { \boldsymbol{c} }
\def \vr { \boldsymbol{r} }
\def \ve{ \boldsymbol{e} }
\def \vW{ \boldsymbol{W} }
\def \vv{ \mathbf{v} }

\def \vsig{ \boldsymbol{\sigma}}
\def \tnsrsig{ \underset{\thickapprox}{\boldsymbol{\sigma} }}
\def \tnsreps{\underset{\thickapprox}{\boldsymbol{\varepsilon} }}
\newcommand{\calp}{\mathbf{p}}
\newcommand{\Erbf}{E_{\rm rbf}}
\def\bicgstab{{BICGSTAB}} 


% ++++ Vectors.
\def \vepsilon{ \boldsymbol{\varepsilon} }
\def \vu{ \boldsymbol{u} }
\def \vU{ \boldsymbol{U} }
\def \vzeta{ \boldsymbol{\zeta} }
\def \vx{ \boldsymbol{x} }
\def \vn{ \boldsymbol{n}}
\def \vf{ \boldsymbol{f} }
\def \vX{ \boldsymbol{X} }
\def \vZ{ \boldsymbol{Z} }
\def \vXd{ \boldsymbol{X}^{\rm d} }
\def \vXs{ \boldsymbol{X}^{\rm s} }
\def \vY{ \boldsymbol{Y} }
\def \vc{ \boldsymbol{c} }
\def \vP{ \boldsymbol{P} }
\def \vF{ \boldsymbol{F} }

% scalars
\def \Xd{ X^{\rm d} }
\def \Xs{ X^{\rm s} }
\def \Yd{ Y^{\rm d} }
\def \Ys{ Y^{\rm s} }
\def \Zd{ Z^{\rm d} }
\def \Zs{ Z^{\rm s} }

\def \Hx { \hat{1} }
\def \Hy { \hat{2} }
\def \Ht{ \hat{t} }
\def \Hu{ \hat{u} }
\def \Hv{ \hat{v} }
\def \Hw{ \hat{w} }
\def \Htau{ \hat{\tau} }

% Grady's commands
\def \ucd{ \vec{c}^X_{\rm d} }
\def \uXd{ \vec{X}_{\rm d}(t) }
\def \uvXd{ \vec{\vX}_{\rm d} }
\def \uvXs{ \vec{\vX}_{\rm s} }
\def \uYd{ \vec{Y}_{\rm d}(t) }
\def \uXs{ \vec{X}_{\rm s}(t) }
\def \uTd{ \vec{T}_{\rm d} }
\def \uvZd{ \vec{\vZ}_{\rm d} }
\def \uvFs{ \vec{\vF}_{\rm s} }
\def \uvFTs{ \vec{\vF}_{\rm s}^{\rm T} }
\def \uvFBs{ \vec{\vF}_{\rm s}^{\rm B} }
\def \uvFCs{ \vec{\vF}_{\rm s}^{\rm C} }
\def \tngtd{ \tngt_{\rm d} }
\def \utngtd{ \vec{\tngt}_{\rm d} }
\def \uutngtd{ \vec{\hat{\tngt}}_{\rm d} }
\def \utngtslon{ \vec{\tngt}_{\rm s}^{\lon} }
\def \utngtslat{ \vec{\tngt}_{\rm s}^{\lat} }
\def \uunrmls{ \vec{\unrml}_{\rm s} }
\def \Es{ \mathcal{E}_{\rm s} }
\def \ub{ \vec{b}_{\lon} }
\def \ubd{ \ub^{n} }
\def \ubs{ \vec{b}_{\lon,\lat} }
\def \ubsd{ \ubs^{m,n} }
\newcommand{\Dlond}[1]{\mathcal{D}_{\lond}^{#1}}
\newcommand{\Dlons}[1]{\mathcal{D}_{\lons}^{#1}}
\newcommand{\Dlonlatd}[2]{\mathcal{D}_{\lond,\latd}^{#1,#2}}
\newcommand{\Dlonlats}[2]{\mathcal{D}_{\lons,\lats}^{#1,#2}}

\def \vhtau{ \boldsymbol{\Htau} }
\def \vc { \boldsymbol{c} }
\def \vn{ \boldsymbol{n} }
\def \vW{ \boldsymbol{W} }
\def \vv{ \mathbf{v} }
\def \vsig{ \boldsymbol{\sigma}}
\def \tnsrsig{ \underset{\thickapprox}{\boldsymbol{\sigma} }}
\def \tnsreps{\underset{\thickapprox}{\boldsymbol{\varepsilon} }}

%  +++++ Tensors
\def \tnsrsig{ \underset{\thickapprox}{\boldsymbol{\sigma} }}
\def \tnsreps{\underset{\thickapprox}{\boldsymbol{\varepsilon} }}

%  +++++ Operators
\def\calB{{\mathcal B}}
\def\calF{{\mathcal F}}
\def\calU{{\mathcal U} }
\def\calUvu{ \mathcal U(\vu) }
\def\calR{\mathcal R }
\def\calS{{ \mathcal S}}
\def\calE{{ \mathcal E}}
\def\calD{{ \mathcal D}}

\newcommand{\Nd}{N_{\rm d}}
\newcommand{\Ns}{N_{\rm s}}
\newcommand{\frcT}{\frc^{\rm T}}
\newcommand{\frcB}{\frc^{\rm B}}
\newcommand{\frcC}{\frc^{\rm C}}
\newcommand{\kt}{k_{\rm t}}
\newcommand{\kb}{k_{\rm b}}
\newcommand{\KC}{K_{\rm C}}
\newcommand{\ellC}{l_{0,\rm C}}

\let\oldenumerate\enumerate
\renewcommand{\enumerate}{
  \oldenumerate
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}

\let\olditemize\itemize
\renewcommand{\itemize}{
  \olditemize
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}

